Actual Knowledge Gain as Privacy Loss in Local Privacy Accounting

This paper establishes the equivalence between Local Differential Privacy (LDP) and a global limit on learning any knowledge specific to a queried object. However, an output from an LDP query is not necessarily required to provide exact amount of knowledge equal to the upper bound of the learning limit. The LDP guarantee can overestimate the amount of knowledge gained by an analyst from some outputs. To address this issue, the least upper bound on the actual knowledge gain is derived and referred to as realized privacy loss. This measure is also shown to serve as an upper bound for the actual g-leakage in quantitative information flow. The gap between the LDP guarantee and realized privacy loss motivates the exploration of a more efficient privacy accounting for fully adaptive composition, where an adversary adaptively selects queries based on prior results. The Bayesian Privacy Filter is introduced to continuously accept queries until the realized privacy loss of the composed queries equals the LDP guarantee of the composition, enabling the full utilization of the privacy budget of an object. The realized privacy loss also functions as a privacy odometer for the composed queries, allowing the remaining privacy budget to accurately represent the capacity to accept new queries. Additionally, a branch-and-bound method is devised to compute the realized privacy loss when querying against continuous values. Experimental results indicate that Bayesian Privacy Filter outperforms the basic composition by a factor of one to four when composing linear and logistic regressions.

==> unused.tex <==
Now we will prove the converse part of the above theorem.

\begin{lemma}
    For a set of queries $M_{\le n}$, if any outputs $y_{\le n}$ from $M_{\le n}$ satisfy $L(y_{\le n}) = \sum\limits_{i = 1}^n \epsilon_i$, and a new query $M_{n+1}$ is not privacy-loss compactible with any queries in $M_{\le n}$, then $L(y_{\le n + 1}) = \sum\limits_{i = 1}^{n+1} \epsilon_i$ for any outputs from $M_{\le n + 1}$.
    % \begin{equation}
    %     \frac{\max\limits_x \prod\limits_x Pr(y_i | x)}{\min\limits_x \prod\limits_x Pr(y_i | x)} = 1
    % \end{equation}
\end{lemma}

\noindent Proof: we will prove it by contradiction. Assume $\exists y_{\le n + 1}: L(y_{\le n + 1}) < \sum\limits_{i = 1}^{n+1} \epsilon_i$. Also assume that $\forall y_{\le n}: L(y_{\le n}) = \sum\limits_{i = 1}^n \epsilon_i$.
\begin{multline}
    \frac{\max\limits_x \prod\limits_{i=1}^{n+1} Pr(y_i | x)}{\min\limits_x \prod\limits_{i=1}^{n+1} Pr(y_i | x)} < \sum\limits_{i = 1}^{n+1} \epsilon_i = \\ \frac{\max\limits_x \prod\limits_{i=1}^{n} Pr(y_i | x)}{\min\limits_x \prod\limits_{i=1}^{n} Pr(y_i | x)}  \frac{\max\limits_x Pr(y_{n+1} | x)}{\min\limits_x Pr(y_{n+1} | x)} .
    \label{eq:K>1_to_compactible_step_1}
\end{multline}

\noindent Either $\max\limits_x \prod\limits_{i=1}^{n+1} Pr(y_i | x) < \max\limits_x \prod\limits_{i=1}^{n} Pr(y_i | x) \allowbreak \max\limits_x Pr(y_{n+1} | x)$ or  $\min\limits_x \prod\limits_{i=1}^{n+1} Pr(y_i | x) > \min\limits_x \prod\limits_{i=1}^{n} \allowbreak Pr(y_i | x) \min\limits_x Pr(y_{n+1} | x)$. We assume the former, while the proof will be similar even if assuming the latter. Define $x_1 \in \argmax_x \prod\limits_{i=1}^{n+1} Pr(y_i | x)$. Also define $\mathbf{x_2} = \allowbreak \argmax_x \prod\limits_{i=1}^{n+1} Pr(y_i | x)$, and $\mathbf{x_3} = \argmax_x Pr(y_{n+1} | x)$, where $\mathbf{x_2}$ and $\mathbf{x_3}$ represent the set of $x$. It is easy to see $\mathbf{x_2} \cap \mathbf{x_3} = \emptyset$. Otherwise, $x_1 \in \mathbf{x_2} \cap \mathbf{x_3}$ and the Eq \eqref{eq:K>1_to_compactible_step_1} will be violated. Given $\forall y_{\le n}: L(y_{\le n}) = \sum\limits_{i = 1}^n \epsilon_i$, we have $\forall x \in \mathbf{x_2}$ is also $\argmax_x Pr(y_j | x)$ where $j \le n$.

Consider $\forall u \in \argmax_x Pr(y_j | x_2) Pr(y_{n+1} | x)$. If $u \in \mathbf{x_2}$, then we have $u \notin \mathbf{x_3}$, so $ \exists y_{n+1}: Pr(y_{n+1} | u) < \max_x Pr(y_{n+1} | x)$. Therefore, we have $\exists y_{n+1}$:
\begin{multline}
    \max\limits_x Pr(y_j | x) Pr(y_{n+1} | x) <  \\ \max\limits_x Pr(y_j | x)  \max\limits_x Pr(y_{n+1} | x).
    \label{eq:K>1_to_compactible_step_2}
\end{multline}

\noindent Consequently,
\begin{multline}
    \frac{\max\limits_x Pr(y_j | x) Pr(y_{n+1} | x)}{\min \limits_x Pr(y_j | x_2) Pr(y_{n+1} | x)} <  \frac{\max\limits_x Pr(y_j | x)  \max\limits_x Pr(y_{n+1} | x)}{\min \limits_x Pr(y_j | x) Pr(y_{n+1} | x)} \\ \le  \frac{\max\limits_x Pr(y_j | x)  \max\limits_x Pr(y_{n+1} | x)}{\min \limits_x Pr(y_j | x) \min \limits_x Pr(y_{n+1} | x)} = e^{\epsilon_j + \epsilon_{n+1}}.
\end{multline}

\noindent Therefore, $M_j$ and $M_{n+1}$ are privacy-loss compactible, which is contradicted to the condition of the Lemma. 

If $u \notin \mathbf{x_2}$, then $u$ cannot be both $\argmax_x \prod_{i = 1, i \ne j}^n Pr(y_i | x)$ and $\argmax_x Pr(y_j | x)$. If $u \notin \argmax_x Pr(y_j | x)$, then Eq. \eqref{eq:K>1_to_compactible_step_2} still holds, so does the consequent contradiction. If $u \notin \argmax_x \prod_{i = 1, i \ne j}^n Pr(y_i | x)$, then
\begin{multline}
    \max\limits_x \prod_{i = 1}^{n+1} Pr(y_i | x) < \\ \max\limits_x \prod_{i = 1, i \ne j}^{n+1} Pr(y_i | x) \max\limits_x [Pr(y_j | x) Pr(y_{n+1} | x)] . 
\end{multline}


\section{Branch and Bound}

Now, we will present the first version of branch-and-bound method (the same procedure as X). Recall that the queries introduced in Section \ref{sec:query_to_dc} requires each dimension of $x \in \mathcal{X}^m$ to have lower and upper bounds, and, for convenience, we call such constraints as a box constraint, denoted as $B^x$. The size of a box constraint is defined to the multiplication of all its lengths (the difference between upper and lower bounds). This method first computes the lower bound of $\min_x \log P(x)$ subject to $B^x$ (denoted as $LB(B^x)$) by solving $f(x) - \sum_i H_i(x)$ using convex optimization. Consider a box constraint $B_i^x$ whose feasible space belongs to that of $B^x$, denoted as $B_i^x \subset B^x$. Based on the definition of a concave envelope, we have $f(x) - \sum_i H_i(x) \rightarrow f(x) - g(x)$ when $\text{size}(B_i^x) \rightarrow 0$. Therefore, the method can converge $LB(B^x)$ to $\min_x \log P(x)$ by continuously split $B^x$ into smaller boxes. To do it, a priority queue is maintained to store all the split boxes. A box with lowest $LB$ will be picked up and split in half against one dimension of the box (i.e. a dimension of $x$). Assume this dimension has a bound of $[l, h]$. Then, the two newly-split boxes will have $[l, \frac{l+h}{2}]$ and $[\frac{l+h}{2}, h]$ as their new bounds of this dimension, while the bounds of other dimensions are unchanged. At the same time, the method computes the upper bound of $\min_x P(x)$ subject to the newly-split box constraint, denoted as $UB(B_i^x)$ where $B_i^x$ is the box constraint. $UB(B_i^x)$ can be acquired by any local optimization of the Difference of Convex Programming (hereinafter referred as LDC algorithm). The LDC algorithms usually utilize Newton Method and/or Sequential Linear Programming to find the local minimum. We choose the DCCP programming \cite{shen2016dccp} as its LDC algorithm. Additionally, the method maintains a global upper bound of $\min_x \log P(x)$ (denoted as $UB_g$) as $\min_{B_i^x \subset B^x}   UB(B_i^x)$. When the $LB$ of a box constraint is above $UB_g$, the method will discard this box without further splitting it. This method continues to run until all the (non-discarded) box constraints have $LB$ close enough to $UB_g$, and outputs $\min LB$ as a good enough lower bound for $\min_x \log P(x)$.

In practice, the $LB$ and $UB_g$ may converge slowly, so this method will be upgraded as follows. Recall that each $f_i(x)$ and $g_i(x)$ can be represented as $F(h(x))$, and denote $y = h(x)$; this gives an heuristic that the change of $f_i(x)$ and $g_i(x)$ is more sensitive to $y$ than $x$. When designing the branch-and-bound method, we could branch (split) on the $y$ of individual queries than $x$. Denote $\mathbf{Y} = \{Y_1, Y_2, ..., Y_n\}$, where $Y_i$ is a variable representing the output of $h_i(x)$. Given $x$ is bounded, each $Y_i$ will have lower and upper bounds, which can be considered as a box constraint on $\mathbf{Y}$, denoted as $B_0^\mathbf{Y}$. The above method is thus upgraded to split $B_0^\mathbf{Y}$ instead. The detail is at Algorithm \ref{algo:BnB}.


\subsection{Quantitative Information Flow}
\label{sec:QIF}
Quantitative Information Flow (QIF) \cite{QIF} uses information theory to study information leakage from a channel (referred to as a query in this paper). QIF considers a leakage as the increase of the vulnerability  of a protected object, and the prior vulnerability before a query is defined as

\begin{equation}
    V(Q) = \max_{x \in \mathcal{X}} Q(X = x) ,
    \notag
\end{equation}

\noindent where $Q$ is the prior belief about $X$. Vulnerability represents the attacker's belief on the likelihood of guessing the actual value. \cite{g-QIF} points out that not only the identity of an object, but also every information about the object, should be protected. Suppose $\mathcal{W}$ is the collection of the information possibly related to object $X$. \cite{g-QIF} proposes a gain function $g(w \in \mathcal{W}, x \in \mathcal{X})$ to measure the relevance between $x$ and $w$. $g(w, x)$ is required to satisfy only $\forall_{x, w} g(x, w) \in [0, 1]$. Different gain functions could have different semantics. Please refer to \cite{g-QIF} for different examples of the gain functions. Given a gain function $g$, we could define the $g$-prior vulnerability of a protected object as

\begin{equation}
    V_g(Q) = \max_w \sum_{x \in \mathcal{X}} Q(x) g(w, x) .
    \notag
\end{equation}

\noindent When a query $M$ is applied against object $X$ and returns $y$, the $g$-posterior vulnerability is defined as

\begin{equation}
    V_g(Q | y) = \max_w \sum_{x \in \mathcal{X}} Q(x | y) g(w, x) .
    \notag
\end{equation}

QIF is focused on the information leakage, and this paper is particularly interested in the actual leakage after a query outputs $y$. Thus, we define the realized $g$-leakage as 

\begin{equation}
    LK_g(Q | y) = \frac{V_g(Q | y)}{V_g(Q)} .
    \notag
\end{equation}
